Scale Free Bounds on the Amplification of Disturbances in Mass Chains

We give a method for designing a mechanical impedance to suppress the propagation of disturbances along a chain of masses. The key feature of our method is that it is scale free. This means that it can be used to give a single, fixed, design, with provable performance guarantees in mass chains of any length. We illustrate the approach by designing a bidirectional control law in a vehicle platoon in a manner that is independent of the number of vehicles in the platoon.

==> Tikz/bode.tex <==
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\begin{tikzpicture}
\pgfplotsset{%
	scaled y ticks=false,
	plot coordinates/math parser=false,
}
\begin{axis}[%
width=0.951\columnwidth,
height=0.5\columnwidth,
at={(0\columnwidth,0\columnwidth)},
scale only axis=true,
xmode=log,
xmin=0.01,
xmax=100,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={{$\omega$ (rad/s)}},
ymode=log,
ymin=0.01,
ymax=1,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={{$|W(j\omega)|f(h(j\omega))$ (dB)}},
%ticklabel style={font=\footnotesize{}},
axis background/.style={fill=white},
xmajorgrids,
xminorgrids,
ymajorgrids,
yminorgrids
]
\addplot [color=mycolor1, forget plot]
  table{Tikz/Data/bode.dat};
\end{axis}
\end{tikzpicture}%

==> Tikz/contour1.tex <==
% This file was created by matlab2tikz v0.4.7 running on MATLAB 7.14.
% Copyright (c) 2008--2014, Nico Schlömer <nico.schloemer@gmail.com>
% All rights reserved.
% Minimal pgfplots version: 1.3
% 
% The latest updates can be retrieved from
%   http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz
% where you can also make suggestions and rate matlab2tikz.
% 
%
% defining custom colors
\definecolor{mycolor1}{rgb}{0.00000,0.00000,0.56250}%
\definecolor{mycolor2}{rgb}{0.00000,0.25000,1.00000}%
\definecolor{mycolor3}{rgb}{0.00000,0.37500,1.00000}%
\definecolor{mycolor4}{rgb}{0.00000,0.50000,1.00000}%
\definecolor{mycolor5}{rgb}{0.00000,0.56250,1.00000}%
\definecolor{mycolor6}{rgb}{0.00000,0.62500,1.00000}%
\definecolor{mycolor7}{rgb}{0.00000,0.68750,1.00000}%
\definecolor{mycolor8}{rgb}{0.00000,0.75000,1.00000}%
\definecolor{mycolor9}{rgb}{0.00000,0.81250,1.00000}%
\definecolor{mycolor10}{rgb}{0.00000,0.87500,1.00000}%
\definecolor{mycolor11}{rgb}{0.12500,1.00000,0.87500}%
\definecolor{mycolor12}{rgb}{0.43750,1.00000,0.56250}%
\definecolor{mycolor13}{rgb}{0.75000,1.00000,0.25000}%
\definecolor{mycolor14}{rgb}{1.00000,0.93750,0.00000}%
\definecolor{mycolor15}{rgb}{1.00000,0.68750,0.00000}%
\definecolor{mycolor16}{rgb}{1.00000,0.06250,0.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=5cm,
height=5cm,
scale only axis,
xmin=-6,
xmax=1,
xlabel={\footnotesize $\mathrm{Re}\funof{z}$},
restrict y to domain*=-10:10,
ymin=-3.25,
ymax=3.25,
ylabel={\footnotesize $\mathrm{Im}\funof{z}$},
colormap/jet,
colorbar,
colorbar style={font=\footnotesize{},ylabel={ $f\funof{z}$ (dB)}},
ticklabel style={font=\footnotesize{}},
point meta min=-20,
point meta max=60
]

\addplot [area legend,solid,fill=mycolor1,draw=none,forget plot]
table {Tikz/Data/contour1/contour1_1.dat};

\addplot[area legend,solid,fill=blue,draw=none,forget plot]
table {Tikz/Data/contour1/contour1_2.dat};

\addplot[area legend,solid,fill=mycolor2,draw=none,forget plot]
table{Tikz/Data/contour1/contour1_3.dat};

\addplot[area legend,solid,fill=mycolor3,draw=none,forget plot]
table {Tikz/Data/contour1/contour1_4.dat};

\addplot[area legend,solid,fill=mycolor4,draw=none,forget plot]
table {Tikz/Data/contour1/contour1_5.dat};


\addplot[area legend,solid,fill=mycolor5,draw=none,forget plot]
table {Tikz/Data/contour1/contour1_6.dat};

\addplot[area legend,solid,fill=mycolor6,draw=none,forget plot]
table {Tikz/Data/contour1/contour1_7.dat};

\addplot[area legend,solid,fill=mycolor7,draw=none,forget plot]
table {Tikz/Data/contour1/contour1_8.dat};


\addplot[area legend,solid,fill=mycolor8,draw=none,forget plot]
table {Tikz/Data/contour1/contour1_9.dat};


\addplot[area legend,solid,fill=mycolor9,draw=none,forget plot]
table{Tikz/Data/contour1/contour1_10.dat};

\addplot[area legend,solid,fill=mycolor9,draw=none,forget plot]
table {Tikz/Data/contour1/contour1_11.dat};


\addplot[area legend,solid,fill=mycolor9,draw=none,forget plot]
table {Tikz/Data/contour1/contour1_12.dat};

\addplot[area legend,solid,fill=mycolor10,draw=none,forget plot]
table {Tikz/Data/contour1/contour1_13.dat};

\addplot[area legend,solid,fill=mycolor11,draw=none,forget plot]
table{Tikz/Data/contour1/contour1_14.dat};

\addplot[area legend,solid,fill=mycolor12,draw=none,forget plot]
table{Tikz/Data/contour1/contour1_15.dat};

\addplot[area legend,solid,fill=mycolor13,draw=none,forget plot]
table {Tikz/Data/contour1/contour1_16.dat};


\addplot[area legend,solid,fill=mycolor14,draw=none,forget plot]
table{Tikz/Data/contour1/contour1_17.dat};

\addplot[area legend,solid,fill=mycolor15,draw=none,forget plot]
table{Tikz/Data/contour1/contour1_18.dat};

\addplot[area legend,solid,fill=red!25!orange,draw=none,forget plot]
table{Tikz/Data/contour1/contour1_19.dat};


\addplot[area legend,solid,fill=mycolor16,draw=none,forget plot]
table {Tikz/Data/contour1/contour1_20.dat};

\addplot[area legend,solid,fill=black!25!red,draw=none,forget plot]
table {Tikz/Data/contour1/contour1_21.dat};

\addplot[area legend,solid,fill=black!50!red,draw=none,forget plot]
table {Tikz/Data/contour1/contour1_22.dat};

\addplot [color=black,solid,line width=2.0pt,forget plot]
  table {Tikz/Data/contour1/contour1_23.dat};
  
\addplot [color=black,solid,line width=2.0pt,forget plot]
  table {Tikz/Data/contour1/contour1_24.dat};
  
\end{axis}
\end{tikzpicture}%

==> Tikz/contour2.tex <==
% This file was created by matlab2tikz v0.4.7 running on MATLAB 7.14.
% Copyright (c) 2008--2014, Nico Schlömer <nico.schloemer@gmail.com>
% All rights reserved.
% Minimal pgfplots version: 1.3
% 
% The latest updates can be retrieved from
%   http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz
% where you can also make suggestions and rate matlab2tikz.
% 
%
% defining custom colors
\definecolor{mycolor1}{rgb}{0.00000,0.00000,0.56250}%
\definecolor{mycolor2}{rgb}{0.00000,0.12500,1.00000}%
\definecolor{mycolor3}{rgb}{0.00000,0.50000,1.00000}%
\definecolor{mycolor4}{rgb}{0.00000,0.87500,1.00000}%
\definecolor{mycolor5}{rgb}{0.25000,1.00000,0.75000}%
\definecolor{mycolor6}{rgb}{0.62500,1.00000,0.37500}%
\definecolor{mycolor7}{rgb}{1.00000,1.00000,0.00000}%
\definecolor{mycolor8}{rgb}{0.87500,0.00000,0.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=5cm,
height=5cm,
colormap/jet,
unbounded coords=jump,
scale only axis,
xmin=-6,
xmax=1,
xlabel={\footnotesize $\mathrm{Re}\funof{z}$},
restrict y to domain*=-10:10,
ymin=-3.24674796747968,
ymax=3.24674796747968,
ylabel={\footnotesize $\mathrm{Im}\funof{z}$},
ticklabel style={font=\footnotesize{}},
colorbar,
colorbar style={font=\footnotesize, ylabel={$\epsilon_n\funof{z}$ (dB)}},
point meta min=0,
point meta max=30
]

\addplot[area legend,solid,fill=mycolor1,draw=none,forget plot]
table {Tikz/Data/contour2/contour2_1.dat};

\addplot[area legend,solid,fill=black!25!blue,draw=none,forget plot]
table {Tikz/Data/contour2/contour2_2.dat};

\addplot[area legend,solid,fill=mycolor2,draw=none,forget plot]
table {Tikz/Data/contour2/contour2_3.dat};

\addplot[area legend,solid,fill=mycolor3,draw=none,forget plot]
table{Tikz/Data/contour2/contour2_4.dat};

\addplot[area legend,solid,fill=mycolor4,draw=none,forget plot]
table{Tikz/Data/contour2/contour2_5.dat};

\addplot[area legend,solid,fill=mycolor5,draw=none,forget plot]
table{Tikz/Data/contour2/contour2_6.dat};

\addplot[area legend,solid,fill=mycolor6,draw=none,forget plot]
table{Tikz/Data/contour2/contour2_7.dat};

\addplot[area legend,solid,fill=orange!75!mycolor7,draw=none,forget plot]
table{Tikz/Data/contour2/contour2_8.dat};

\addplot[area legend,solid,fill=red!50!orange,draw=none,forget plot]
table{Tikz/Data/contour2/contour2_9.dat};

\addplot[area legend,solid,fill=mycolor8,draw=none,forget plot]
table {Tikz/Data/contour2/contour2_10.dat};

\addplot[area legend,solid,fill=black!50!red,draw=none,forget plot]
table {Tikz/Data/contour2/contour2_11.dat};

\addplot[area legend,solid,line width=2.0pt,draw=white,forget plot]
table{Tikz/Data/contour2/contour2_12.dat};

\end{axis}
\end{tikzpicture}%

==> Tikz/platoon_disp.tex <==
\begin{tikzpicture}
\pgfplotsset{%
	scaled y ticks=false,
	plot coordinates/math parser=false,
}
\begin{axis}[%
	width=0.951\columnwidth,
	height=0.5\columnwidth,
	at={(0\columnwidth,0\columnwidth)},
	scale only axis,
	xmin=0,
	xmax=1000,
	xlabel style={font=\color{white!15!black}},
	xlabel={{time (seconds)}},
	ymin=-0.03,
	ymax=0.05,
	ylabel style={font=\color{white!15!black}},
	ylabel={{$\hat{x}_0(t)-\hat{x}_1(t)$}},
	yticklabel style={
			/pgf/number format/fixed,
			/pgf/number format/precision=3
	},
	%ticklabel style={font=\footnotesize{}},
	axis background/.style={fill=white},
	xmajorgrids,
	ymajorgrids,
	legend style={legend cell align=left, align=left, draw=white!15!black, font=\footnotesize{}}
]
	\addplot [color=blue, line width=1.0pt] table{Tikz/Data/N10.dat};
	\addlegendentry{$N=10$}

	\addplot [color=red, dotted, line width=1.0pt] table{Tikz/Data/N30.dat};
	\addlegendentry{$N=30$}

	\addplot [color=black, dashed, line width=1.0pt] table{Tikz/Data/N100.dat};
	\addlegendentry{$N=100$}
\end{axis}
\end{tikzpicture}%
